Diffusion Language Models Are Versatile Protein Learners

This paper introduces diffusion protein language model (DPLM), a versatile protein language model that demonstrates strong generative and predictive capabilities for protein sequences. We first pre-train scalable DPLMs from evolutionary-scale protein sequences within a generative self-supervised discrete diffusion probabilistic framework, which generalizes language modeling for proteins in a principled way. After pre-training, DPLM exhibits the ability to generate structurally plausible, novel, and diverse protein sequences for unconditional generation. We further demonstrate the proposed diffusion generative pre-training makes DPLM possess a better understanding of proteins, making it a superior representation learner, which can be fine-tuned for various predictive tasks, comparing favorably to ESM2 (Lin et al., 2022). Moreover, DPLM can be tailored for various needs, which showcases its prowess of conditional generation in several ways: (1) conditioning on partial peptide sequences, e.g., generating scaffolds for functional motifs with high success rate; (2) incorporating other modalities as conditioner, e.g., structure-conditioned generation for inverse folding; and (3) steering sequence generation towards desired properties, e.g., satisfying specified secondary structures, through a plug-and-play classifier guidance. Code is released at \url{https://github.com/bytedance/dplm}.

==> tables/inverse_folding.tex <==
% \begin{table*}[t]
%    \centering
%    \small
%    % \setlength{\tabcolsep}{5pt}
%    \vspace{-2.5mm}
%    \caption{{\sl Performance comparison between \method and different baseline approaches on CATH 4.2 and CATH 4.3 datasets.} {\method's results are obtained by 5-cycle iterative refinement with \texttt{argmax} operator (\ie, no sampling).}
%    $\dagger$: benchmarked results are quoted from \citet{gao2022pifold}.
%    $\ddagger$: ``Single-chain'' in \citet{hsu2022esmif} is defined differently. ESM-1b 650M is used as the default \pLM.}
%    \vspace{1.5pt}
%    \label{tab:inverse_folding}

%    \resizebox{\linewidth}{!}{%
%    \begin{tabular}{llrccc}
%    \toprule
%    & \multirow{2}{*}{\bf Models} 
%    & \multirow{2}{*}{\bf Trainable/Total} 
%    & \multicolumn{1}{c}{\bf Sequence Metric ($\uparrow$)} 
%    & \multicolumn{2}{c}{\bf Structure Metric (\%, $\uparrow$)} \\
%    \cmidrule[0.3pt](lr){4} \cmidrule[0.3pt](lr){5-6}
%    & & \bf Params. & AAR   & scTMscore  & pLDDT \\
%    \midrule
%    % StructGNN &  8.29   &   8.74   &  6.40 &   29.44 &   28.26   &  35.91   \\

%    %%%%%%%%%%%%%%%%%%%%%%%%%%
%    \multirowcell{10}{\rotatebox[origin=c]{90}{CATH 4.2}}
%    & $^\dagger$Structured Transformer~\smallcitep{ingraham2019generative}                     & 1.56M/1.56M  & 8.39  & 8.83 & 6.63 \\
%    % & GCA&  7.09&  7.49  &  6.05  & 32.62 & 31.10 & 37.64 \\
%    & $^\dagger$GVP~\smallcitep{jing2020gvp}                                       & 1.0M/1.0M  & 7.23  &   7.84 &  5.36  \\
%    % & AlphaDesign &  7.32  & 7.63 &  6.30 &  34.16  & 32.66  &  41.31   \\
%    & $^\dagger$ProteinMPNN~\smallcitep{dauparas2022proteinmpnn}                   & 1.9M/1.9M  & 6.21  &   6.68  &  4.61  \\
%    & PiFold~\smallcitep{gao2022pifold} \                                & 6.6M/6.6M  & {6.04}  &   {6.31}  &  {4.55}  \\ 
%   %%%%%%%%%%%%%%% OURS %%%%%%%%%%%%%%%%%%%
%   \cmidrule[0.5pt](lr){2-9}
%   & ProteinMPNN + CMLM [ProtMPNN-CMLM]                                                 & 1.9M/1.9M  &7.16 &7.25  & 5.03     \\ 
%   & \chl \method (ProtMPNN-CMLM)                                          & \chl 6.9M/659M (\textbf{1.0\%})  &\chl 7.02 & \chl 6.67 & \chl 4.63    \\ 
%   & \chl \method (pretrained ProtMPNN-CMLM: \textit{fine-tune})           & \chl 6.9M/659M (\textbf{1.0\%})  & \chl 7.33 & \chl 6.83 & \chl 4.63  \\
%   & \chl \method (pretrained ProtMPNN-CMLM: \textit{freeze})              & \chl 5.0M/659M (\textbf{0.7\%})  & \chl \textbf{7.01} & \chl \textbf{6.58} & \chl \textbf{4.41} \\
%   \cmidrule[0.2pt](lr){2-9}
%   & PiFold (reimpl.)                                                    & 6.6M/6.6M  & 6.94 &6.82  &4.69   \\ 
%   & \chl \method (PiFold)                                               & \chl 11.9M/664M (\textbf{1.7\%})  & \chl \textbf{6.77} & \chl \textbf{6.46}   & \chl \textbf{4.52}   \\ 
%   \midrule
%   % \cmidrule[0.5pt](lr){2-8}

%   %%%%%%%%%%%%%%%%%%%%%%%%%%
%   \multirowcell{10}{\rotatebox[origin=c]{90}{CATH 4.3}}
%   & GVP-large~\citep{hsu2022esmif}                                      & 21M/21M  &  7.68  & $^\ddagger$6.12~~ &  6.17   \\
%   & GVP-Transformer~\citep{hsu2022esmif}                                 & 142M/142M  &   8.18 & $^\ddagger$6.33~~ &  6.44  \\
%   & ~~~~+1.2M AF2 predicted data~\smallcitep{hsu2022esmif}              & 142M/142M  &   6.05 & $^\ddagger$4.00~~ &  4.01 \\
%   & \chl \method (pretrained GVP-TransEncoder: \textit{freeze})          & \chl 6.3M/800M (\textbf{0.8\%})  & \chl 6.61 & \chl 7.64 & \chl \textbf{3.92} \\
%   % & PiFold~\smallcitep{gao2022pifold} \   &  {6.04}  &   {6.31}  &  {4.55} &   {39.84} &{38.53} &  {51.66} \\ 
%   %%%%%%%%%%%%%%% OURS %%%%%%%%%%%%%%%%%%%
%   \cmidrule[0.5pt](lr){2-9}
%   & ProteinMPNN + CMLM                                                  & 1.9M/1.9M  & 6.31 &6.32  &4.85      \\ 
%   & \chl \method (ProtMPNN-CMLM)                                          & \chl 6.9M/659M (\textbf{1.0\%})  & \chl 5.96 &\chl 5.85 &\chl 4.48    \\ 
%   & \chl \method (pretrained ProtMPNN-CMLM: \textit{fine-tune})           & \chl 6.9M/659M (\textbf{1.0\%})  & \chl 5.94 & \chl 5.80 & \chl 4.20  \\
%   & \chl \method (pretrained ProtMPNN-CMLM: \textit{freeze})              & \chl 5.0M/659M (\textbf{0.7\%})  & \chl \textbf{5.88} & \chl \textbf{5.66} & \chl \textbf{4.19}  \\
%   \cmidrule[0.2pt](lr){2-9}
%   & PiFold (reimpl.)                                                    & 6.6M/6.6M  & 5.88& 5.55 & 4.47   \\ 
%   & \chl \method (PiFold)                                               & \chl 11.9M/664M (\textbf{1.7\%})  &\chl \textbf{5.66} &\chl \textbf{5.52}  &\chl 4.01  \\ 
  
%    \bottomrule
%    \end{tabular}
%    }
%    % \vspace{-8pt}
% \end{table*}



=========================
% \begin{table*}[]
% \begin{tabular}{lllll}
% \hline
%                             & Params & AAR & scTMscore & pLDDT          \\ \hline
% PiFold                      & 6.6M                           & 50.68                       & TODO                              & TODO           \\
% GRADE-IF                    & -                              & TODO                        & TODO                              & TODO           \\
%                             & 150m                           & 53.08                       & 0.84                              & 74.40          \\
% \multirow{-2}{*}{LM-DESIGN} & 650m                           & \textbf{56.69}              & 0.85                              & 74.89          \\
%                             & 150m                           & \textbf{53.27}              & 0.84                              & 73.84          \\
% \multirow{-2}{*}{\chl DIFF-LM}   & 650m                           & 56.36                       & \textbf{0.8575}                   & \textbf{76.94} \\ \hline
% \end{tabular}
% \end{table*}

==> tables/motif_omegafold.tex <==
\begin{table}[t!]
   \centering
   \small
   \setlength{\tabcolsep}{2pt}
   \vspace{-3mm}
   \caption{{\sl Performance comparison between \method and different baseline approaches on CATH 4.2 and CATH 4.3 datasets.}
   {\method's results are obtained by \texttt{argmax} decoding (\ie, no sampling).}
   $\dagger$: benchmarked results are quoted from \citet{gao2022pifold}.
   }
   % \vspace{1.5pt}
   \label{tab:results_cath}

   \resizebox{\linewidth}{!}{%
   \begin{tabular}{llrccc}
   \toprule
   & \multirow{2}{*}{ Models} 
   & \multirow{2}{*}{ Trainable} 
   & \multirow{2}{*}{\metric{AAR}} 
   & \multicolumn{2}{c}{\bf struct. eval.} \\
    \cmidrule[0.3pt](lr){5-6} & & \bf Params. & & \metric{scTM}  & \metric{pLDDT} \\
   \midrule
   % StructGNN &  8.29   &   8.74   &  6.40 &   29.44 &   28.26   &  35.91   \\

   %%%%%%%%%%%%%%%%%%%%%%%%%%
   \multirowcell{7}{\rotatebox[origin=c]{90}{CATH 4.2}}
   & $^\dagger$StructTrans~\smallcitep{ingraham2019generative}                     & 1.6M/1.6M  & 35.82&   -   & - \\
   % & GCA&  7.09&  7.49  &  6.05  & 32.62 & 31.10 & 37.64 \\
   & $^\dagger$GVP~\smallcitep{jing2020gvp}                                       & 1.0M/1.0M  &  39.47 &   - & -  \\
   % & AlphaDesign &  7.32  & 7.63 &  6.30 &  34.16  & 32.66  &  41.31   \\
   & $^\dagger$ProteinMPNN~\smallcitep{dauparas2022proteinmpnn}                   & 1.9M/1.9M  &  45.96 &  -  & -    \\
   & PiFold~\smallcitep{gao2022pifold} \                                        & 6.6M/6.6M  &  {51.66} &   {-} &{-}  \\ 
  %%%%%%%%%%%%%%% OURS %%%%%%%%%%%%%%%%%%%
  \cmidrule[0.5pt](lr){2-6}
  & ProteinMPNN + CMLM                                                 & 1.9M/1.9M  &48.62     & - & - \\ 
  % & \chl \method (ProtMPNN-CMLM)                                          & \chl 6.9M/659M (\textbf{1.0\%})  &\chl 7.02 & \chl 6.67 & \chl 4.63   & \chl 35.71  & \chl 38.61 & \chl 53.26 \\ 
  % & \chl \method (pretrained ProtMPNN-CMLM: \textit{fine-tune})           & \chl 6.9M/659M (\textbf{1.0\%})  & \chl 7.33 & \chl 6.83 & \chl 4.63 & \chl \textbf{36.47} & \chl \textbf{40.91} & \chl \textbf{54.62} \\
  % \cmidrule[0.2pt](lr){2-9}
  % & PiFold (reimpl.)                                                    & 6.6M/6.6M  &50.22  &- &-   \\ 

  &  \textsc{LM-Design} (\textit{w/} ProtMPNN encoder)              &  5.0M/659M   &  {54.41} &  0.88 &  77.07 \\
  & \chl \method (\textit{w/} ProtMPNN encoder)              & \chl 5.0M/659M   & \chl \textbf{54.54} & \chl 0.88 & \chl \textbf{77.12} \\
  \midrule
  % \cmidrule[0.5pt](lr){2-8}

  %%%%%%%%%%%%%%%%%%%%%%%%%%
  \multirowcell{4}{\rotatebox[origin=c]{90}{CATH 4.3}}
  & PiFold~\smallcitep{gao2022pifold} & 6.6M/6.6M    &  {51.66} & - & - \\ 
  & GVP-Transformer~\citep{hsu2022esmif}                                 & 142M/142M  &  51.60 &   - & -  \\
  &  \textsc{LM-Design} (\textit{w/} GVP-Trans encoder)          &  3.1M/302M  & 53.08 &  0.84 & 74.40  \\
  &  \textsc{LM-Design} (\textit{w/} GVP-Trans encoder)          &  6.3M/800M  & 56.49 &  0.85 & 74.89  \\
  %%%%%%%%%%%%%%% OURS %%%%%%%%%%%%%%%%%%%
  \cmidrule[0.5pt](lr){2-6}
  % & ProteinMPNN + CMLM                                                  & 1.9M/1.9M  & 6.31 &6.32  &4.85     & 40.30 & 39.02 &  48.25  \\ 
  % & \chl \method (ProtMPNN-CMLM)                                          & \chl 6.9M/659M (\textbf{1.0\%})  & \chl 5.96 &\chl 5.85 &\chl 4.48   & \chl 44.12  & \chl 44.05 &\chl 54.05 \\ 
  % & \chl \method (pretrained ProtMPNN-CMLM: \textit{fine-tune})           & \chl 6.9M/659M (\textbf{1.0\%})  & \chl 5.94 & \chl 5.80 & \chl 4.20 & \chl 45.65 & \chl \textbf{46.15} & \chl 55.92 \\
  % & \chl \method (pretrained ProtMPNN-CMLM: \textit{freeze})              & \chl 5.0M/659M (\textbf{0.7\%})  & \chl \textbf{5.88} & \chl \textbf{5.66} & \chl \textbf{4.19} & \chl \textbf{45.71} & \chl \textbf{46.15} & \chl \textbf{56.38} \\
  % \cmidrule[0.2pt](lr){2-9}
  % & PiFold (reimpl.)                                                    & 6.6M/6.6M  & 5.88& 5.55 & 4.47  & 42.86 &43.69& 50.68    \\ 
  & \chl \method (\textit{w/} GVP-Trans encoder)                                               & \chl 3.1M/302M   &\chl \textbf{53.27}   & \chl \textbf{0.85}  &\chl \textbf{75.31}  \\ 
  & \chl \method (\textit{w/} GVP-Trans encoder)                                               & \chl 6.3M/800M   &\chl \textbf{56.61}   & \chl \textbf{0.86}  &\chl \textbf{76.78}  \\ 
  
\bottomrule
\end{tabular}
}
   % \vspace{-8pt}
\end{table}

